Multi-task Learning over Graph Structures

We present two architectures for multi-task learning with neural sequence models. Our approach allows the relationships between different tasks to be learned dynamically, rather than using an ad-hoc pre-defined structure as in previous work. We adopt the idea from message-passing graph neural networks and propose a general \textbf{graph multi-task learning} framework in which different tasks can communicate with each other in an effective and interpretable way. We conduct extensive experiments in text classification and sequence labeling to evaluate our approach on multi-task learning and transfer learning. The empirical results show that our models not only outperform competitive baselines but also learn interpretable and transferable patterns across tasks.

==> AAAI-Multi-task Communication/commands.tex <==
% Packages hyperref and algorithmic misbehave sometimes.  We can fix
% this with the following command.
%\newcommand{\theHalgorithm}{\arabic{algorithm}}
\DeclareMathOperator*{\GraphSen}{GraphSen}
\DeclareMathOperator*{\TreeLSTM}{TreeLSTM}
\DeclareMathOperator*{\GraphLSTM}{GraphLSTM}
\DeclareMathOperator*{\RN}{RN}
\DeclareMathOperator*{\InraAtt}{InraAtt}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\MOD}{MOD}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand\newcite[1]{\citeauthor{#1} [\citeyear{#1}]}
\DeclareMathOperator*{\softmax}{softmax}
\DeclareMathOperator*{\ff}{f}
\newcommand{\bs}[1]{\boldsymbol{\mathbf{#1}}}
\def\W{\mathbf{W}}
\def\U{\mathbf{U}}
\def\bb{\mathbf{b}}

\def\bx{\mathbf{x}}
\def\bh{\mathbf{h}}
\def\bH{\mathbf{H}}
\def\V{\mathbf{V}}
\def\e{\mathbf{e}}
\def\a{\mathbf{a}}
\def\h{\mathbf{h}}
\def\rr{\mathbf{r}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\cc{\mathbf{c}}
\def\ii{\mathbf{i}}
\def\ff{\mathbf{f}}
\def\oo{\mathbf{o}}
\def\u{\mathbf{u}}
\def\g{\mathbf{g}}
\def\p{\mathbf{p}}
\def\q{\mathbf{q}}
\def\bt{\mathbf{t}}
\def\SS{\mathbf{S}}
%\def\s{\mathbf{s}}
\def\ss{\mathbf{s}}
\def\cc{\mathbf{c}}
\def\bw{\mathbf{w}}
\def\H{\mathbf{H}}
\def\P{\mathbf{P}}
\def\R{\mathbb{R}}
\def\l{\mathbf{l}}
\def\M{\mathbf{M}}
\def\w{\mathbf{w}}
\def\W{\mathbf{W}}
\def\U{\mathbf{U}}
\def\bb{\mathbf{b}}
\def\y{\mathbf{y}}
\def\V{\mathbf{V}}
\def\e{\mathbf{e}}
\def\h{\mathbf{h}}
\def\rr{\mathbf{r}}
\def\x{\mathbf{x}}
\def\cc{\mathbf{c}}
\def\ii{\mathbf{i}}
\def\ff{\mathbf{f}}
\def\oo{\mathbf{o}}
\def\u{\mathbf{u}}
\def\g{\mathbf{g}}



% meta-learning stuff
\newcommand{\be}{\mathbf{e}}
\newcommand{\task}{\mathcal{T}}
\newcommand{\bigloss}{\mathcal{L}}
\newcommand{\loss}{\ell}
\newcommand{\inp}{\mathbf{x}}
\newcommand{\inpbias}{\check{\mathbf{x}}} % input with bias transformation
\newcommand{\out}{\mathbf{y}}
\newcommand{\act}{\mathbf{a}}
\newcommand{\learner}{f}
\newcommand{\error}{\mathbf{e}}
\newcommand{\policy}{\pi}
\newcommand{\dataset}{\mathcal{D}}
\newcommand{\rnn}{g}
\newcommand{\gd}{h}
\newcommand{\testinp}{\inp^\star}
\newcommand{\testout}{\hat{\out}^\star}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bzt}{\tilde{\mathbf{z}}}
\newcommand{\bzb}{\overline{\mathbf{z}}}
\newcommand{\ro}{f_{\text{out}}}
\newcommand{\nn}{\hat{f}}
\newcommand{\ft}{\tilde{\phi}}
\newcommand{\Wt}{\tilde{W}}
\newcommand{\Wb}{\overline{W}}
\newcommand{\eb}{\overline{e}}
\newcommand{\et}{\tilde{e}}
\newcommand{\Mt}{\tilde{M}}
\newcommand{\Mb}{\overline{M}}
\newcommand{\ftparams}{\theta_\text{ft}}
\newcommand{\hpost}{h_\text{post}}
% Employ the following version of the ``usepackage'' statement for
% submitting the draft version of the paper for review.  This will set
% the note in the first column to ``Under review.  Do not distribute.''
%\usepackage{icml2017}

% Employ this version of the ``usepackage'' statement after the paper has
% been accepted, when creating the final version.  This will set the
% note in the first column to ``Proceedings of the...''
%\usepackage[accepted]{icml2017}

\newenvironment{itemize*}%
 {\begin{itemize}%
  \setlength{\itemsep}{0pt}%
  \setlength{\parskip}{0pt}}%
 {\end{itemize}}
 \newenvironment{enumerate*}%
 {\begin{enumerate}%
  \setlength{\itemsep}{0pt}%
  \setlength{\parskip}{0pt}}%
 {\end{enumerate}}


\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
%\SetCommentSty{mycommfont}
\newcommand\BibTeX{B{\sc ib}\TeX}

==> commands.tex <==
% Packages hyperref and algorithmic misbehave sometimes.  We can fix
% this with the following command.
%\newcommand{\theHalgorithm}{\arabic{algorithm}}
\DeclareMathOperator*{\GraphSen}{GraphSen}
\DeclareMathOperator*{\TreeLSTM}{TreeLSTM}
\DeclareMathOperator*{\GraphLSTM}{GraphLSTM}
\DeclareMathOperator*{\RN}{RN}
\DeclareMathOperator*{\InraAtt}{InraAtt}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\MOD}{MOD}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%\newcommand\newcite[1]{\citeauthor{#1} [\citeyear{#1}]}
\DeclareMathOperator*{\softmax}{softmax}
\DeclareMathOperator*{\ff}{f}
\newcommand{\bs}[1]{\boldsymbol{\mathbf{#1}}}
\def\W{\mathbf{W}}
\def\U{\mathbf{U}}
\def\bb{\mathbf{b}}

\def\bx{\mathbf{x}}
\def\bh{\mathbf{h}}
\def\bH{\mathbf{H}}
\def\V{\mathbf{V}}
\def\e{\mathbf{e}}
\def\a{\mathbf{a}}
\def\h{\mathbf{h}}
\def\rr{\mathbf{r}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\cc{\mathbf{c}}
\def\ii{\mathbf{i}}
\def\ff{\mathbf{f}}
\def\oo{\mathbf{o}}
\def\u{\mathbf{u}}
\def\g{\mathbf{g}}
\def\p{\mathbf{p}}
\def\q{\mathbf{q}}
\def\bt{\mathbf{t}}
\def\SS{\mathbf{S}}
%\def\s{\mathbf{s}}
\def\ss{\mathbf{s}}
\def\cc{\mathbf{c}}
\def\bw{\mathbf{w}}
\def\H{\mathbf{H}}
\def\P{\mathbf{P}}
\def\R{\mathbb{R}}
\def\l{\mathbf{l}}
\def\M{\mathbf{M}}
\def\w{\mathbf{w}}
\def\W{\mathbf{W}}
\def\U{\mathbf{U}}
\def\bb{\mathbf{b}}
\def\y{\mathbf{y}}
\def\V{\mathbf{V}}
\def\e{\mathbf{e}}
\def\h{\mathbf{h}}
\def\rr{\mathbf{r}}
\def\x{\mathbf{x}}
\def\cc{\mathbf{c}}
\def\ii{\mathbf{i}}
\def\ff{\mathbf{f}}
\def\oo{\mathbf{o}}
\def\u{\mathbf{u}}
\def\g{\mathbf{g}}



% meta-learning stuff
\newcommand{\be}{\mathbf{e}}
\newcommand{\task}{\mathcal{T}}
\newcommand{\bigloss}{\mathcal{L}}
\newcommand{\loss}{\ell}
\newcommand{\inp}{\mathbf{x}}
\newcommand{\inpbias}{\check{\mathbf{x}}} % input with bias transformation
\newcommand{\out}{\mathbf{y}}
\newcommand{\act}{\mathbf{a}}
\newcommand{\learner}{f}
\newcommand{\error}{\mathbf{e}}
\newcommand{\policy}{\pi}
\newcommand{\dataset}{\mathcal{D}}
\newcommand{\rnn}{g}
\newcommand{\gd}{h}
\newcommand{\testinp}{\inp^\star}
\newcommand{\testout}{\hat{\out}^\star}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bzt}{\tilde{\mathbf{z}}}
\newcommand{\bzb}{\overline{\mathbf{z}}}
\newcommand{\ro}{f_{\text{out}}}
\newcommand{\nn}{\hat{f}}
\newcommand{\ft}{\tilde{\phi}}
\newcommand{\Wt}{\tilde{W}}
\newcommand{\Wb}{\overline{W}}
\newcommand{\eb}{\overline{e}}
\newcommand{\et}{\tilde{e}}
\newcommand{\Mt}{\tilde{M}}
\newcommand{\Mb}{\overline{M}}
\newcommand{\ftparams}{\theta_\text{ft}}
\newcommand{\hpost}{h_\text{post}}
% Employ the following version of the ``usepackage'' statement for
% submitting the draft version of the paper for review.  This will set
% the note in the first column to ``Under review.  Do not distribute.''
%\usepackage{icml2017}

% Employ this version of the ``usepackage'' statement after the paper has
% been accepted, when creating the final version.  This will set the
% note in the first column to ``Proceedings of the...''
%\usepackage[accepted]{icml2017}

\newenvironment{itemize*}%
 {\begin{itemize}%
  \setlength{\itemsep}{0pt}%
  \setlength{\parskip}{0pt}}%
 {\end{itemize}}
 \newenvironment{enumerate*}%
 {\begin{enumerate}%
  \setlength{\itemsep}{0pt}%
  \setlength{\parskip}{0pt}}%
 {\end{enumerate}}


\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
%\SetCommentSty{mycommfont}
\newcommand\BibTeX{B{\sc ib}\TeX}
